Efficient Parallel Ising Samplers via Localization Schemes

We introduce efficient parallel algorithms for sampling from the Gibbs distribution and estimating the partition function of Ising models. These algorithms achieve parallel efficiency, with polylogarithmic depth and polynomial total work, and are applicable to Ising models in the following regimes: (1) Ferromagnetic Ising models with external fields; (2) Ising models with interaction matrix $J$ of operator norm $\|J\|_2<1$. Our parallel Gibbs sampling approaches are based on localization schemes, which have proven highly effective in establishing rapid mixing of Gibbs sampling. In this work, we employ two such localization schemes to obtain efficient parallel Ising samplers: the \emph{field dynamics} induced by \emph{negative-field localization}, and \emph{restricted Gaussian dynamics} induced by \emph{stochastic localization}. This shows that localization schemes are powerful tools, not only for achieving rapid mixing but also for the efficient parallelization of Gibbs sampling.

==> sec/good-event.tex <==
\subsection{Application on random cluster model at low temperature (proof of \Cref{thm:GD-correctness})} \label{sec:verify-cond-GD-sim}

% In this section, we prove \Cref{lemma:verify-cond-GD-sim}.
% We need to verify \Cref{cond:good-event-property} under the assumptions of \Cref{thm:GD-correctness}.
% Recall that we have $n = \abs{V} \geq 3$, $0 < \epsilon \leq 1/2$, and $\*p \geq 1 - K/\log n$, where
% \begin{align*}
%     K \leq \min\left\{\-{e}^{-40} \exp\tp{-\frac{5\log (1/\epsilon)}{\log n}}, \frac{1 - \lambda_{\max}}{27} \right\}
%     \text{ and }
%     T^{\-{GD}} = \ctp{2m(\log m + \log(4/\epsilon))}.
% \end{align*}

% {\color{red}
Recall that $G = (V, E)$, $\*p, \*\lambda$, and $\epsilon$ are the input of \Cref{alg:BP-simulation}, where it holds that $n=\abs{V} \geq 3$, $\epsilon \leq 1/2$, and 
    \begin{align*}
        (1-p_{\min}) \log n \leq \min\left\{\-{e}^{-40} \exp\tp{-\frac{5\log (1/\epsilon)}{\log n}}, \frac{1 - \lambda_{\max}}{27} \right\}.
\end{align*}
Furthermore, $T^{\-{GD}} \ge \ctp{2m(\log m + \log(4/\epsilon))}$ and $\tPA \ge \lceil 3\log \left( 4\tGD/\epsilon \right) \rceil$ are parameters used in \cref{alg:BP-simulation}.
These assumptions will be used throughout.
% }


First, under the above assumption, it is known that
the Glauber dynamics for the distribution $\mu = \mu^{\-RC}_{E, \*p, \*\lambda}$ of the random cluster model is rapidly mixing.
%We have the following results for proving \Cref{thm:GD-correctness}.

\begin{lemma}[\text{\cite[Theorem 5.1]{chen2023nearlinear}}] \label{lemma:GD-mixing}
Let $(X_i)_{i=0}^{\tGD}$ be the Glauber dynamics on the distribution $\mu$ with the initial state $X_0$ generated as in \cref{line:ini-X} of \cref{alg:BP-simulation},
%Let $G = (V, E)$, $\*p, \*\lambda$, and $\epsilon$ be the input of \Cref{alg:BP-simulation}. 
%Furthermore, let $\tGD = \ctp{2m(\log m + \log(4/\epsilon))}$ be the length of process $(X_i)_{i=0}^{\tGD}$ and the initial state $X_0$ is the random configuration generated in \cref{line:ini-X} of \cref{alg:BP-simulation}.
%    If $n=|V|\ge 3$, $\epsilon \leq\frac{1}{2}$ and
%    \begin{align*}
%        (1 - p_{\min}) \log n &\leq \min\left\{\-{e}^{-40} \exp\tp{-\frac{5\log (1/\epsilon)}{\log n}}, \frac{1 - \lambda_{\max}}{27} \right\},
%    \end{align*}
    then it holds that $$\DTV{X_{T^{\-{GD}}}}{\mu} \leq \epsilon / 2.$$
\end{lemma}

\begin{remark}
In~\cite{chen2023nearlinear}, the initial state of the Glauber dynamics was set to $E$ instead of the random $X_0$. Though, the proof of~\cite[Theorem 5.1]{chen2023nearlinear} holds so long as the initial state follows the law of a product distribution whose marginal probabilities are bounded from below by $1-3(1-p_{\min})\log n$. By the argument in~\cite[Lemma 5.5]{chen2023nearlinear}, this is satisfied by the random initial state $X_0$ in \Cref{lemma:GD-mixing}. 
\end{remark}

We are now ready to prove \Cref{thm:GD-correctness}.
\begin{proof}[Proof of \Cref{thm:GD-correctness}]
% Since we assume $\epsilon \leq 1/2$, our choice of $K$ implies that
% \begin{align*}
%      K \leq \min\left\{10^{-5} \exp\tp{-\frac{\log (16/\epsilon)}{\log n}}, \frac{1 - \lambda_{\max}}{27} \right\},
% \end{align*}
% which meets the requirements in \Cref{lemma:GD-mixing}.
% {\color{red}
We first prove \Cref{thm:GD-correctness} by assuming \Cref{cond:good-event-property} with parameter $\eta = \frac{\epsilon}{16 \tGD}$.
By \cref{thm:dtv-xALG-GD} and the assumption of parameters, 
\begin{align*}
    \DTV{\xALG}{X_{\tGD}} \le 2\tGD \cdot 2^{- 3\log (4\tGD/\epsilon)} + 4\tGD \cdot \frac{\epsilon}{16\tGD} \le \epsilon / 2.
\end{align*}
Therefore, by \Cref{lemma:GD-mixing} and a triangle inequality, it holds that
\begin{align*}
    \DTV{\xALG}{\mu} &\leq \DTV{\xALG}{\xGD} + \DTV{\xGD}{\mu} \leq \epsilon. 
\end{align*}
% }
The remaining proof is dedicated to verifying \cref{cond:good-event-property} with parameter $\eta = \frac{\epsilon}{16\tGD}$.
% By \Cref{lemma:GD-mixing}, \Cref{thm:dtv-xALG-GD}, \Cref{lemma:verify-cond-GD-sim}, and a triangle inequality, it holds that
% \begin{align*}
%     \DTV{\xALG}{\mu} &\leq \DTV{\xALG}{\xGD} + \DTV{\xGD}{\mu} \leq \epsilon. \qedhere
% \end{align*}


% Now, to prove \Cref{thm:GD-correctness}, it is sufficient for us to verify \Cref{cond:good-event-property}.

\paragraph*{Verifying \Cref{item:good-event-1} of \Cref{cond:good-event-property}:} let $\+C$ be the family of vertex sets with large expansion:
\begin{align*}
    \+C := \left\{ S \subseteq V \mid  \abs{S} \leq n/2 \text{ and } \abs{E(S, V\setminus S)} \geq \abs{S} \log n \right\},
\end{align*}
where $E(S, V\setminus S)$ is the set of edges between $S$ and $V\setminus S$. 
We define the good event
\begin{align*}
    \+G := \left\{X\subseteq E \mid \forall S\in \+C, \abs{X \cap E(S, V\setminus S)} > 0 \right\}.
\end{align*}
We remark that this is the same good event used in \cite[Section 5]{chen2023nearlinear}.
%In \cite[Equation 8]{chen2023nearlinear}, it has been shown that for every $X, Y \in \+G$ with $X \oplus Y = \{f\}$,
%\begin{align*}
%    1 - \frac{1}{m} + \frac{1}{m} \sum_{e \in E\setminus \{f\}} \abs{\mu^X_e - \mu^Y_e} \leq 1 - \frac{1}{2m}.
%\end{align*}
%{\color{red}
In has been established in \cite[Eq.~(14)]{chen2023nearlinear} that
\begin{align*}
    \sum_{e \in E \setminus\{f\}} \abs{\mu^X_e - \mu^Y_e} = 0.
\end{align*}
%}
Note that we also have $\abs{\mu^X_f - \mu^Y_f} = 0$ by definition. Therefore,
\begin{align} \label{eq:1-dist-decay}
    \sum_{e \in E} \abs{\mu^X_e - \mu^Y_e} \leq \frac{1}{2}.
\end{align}
For $X, Y \in \+G$ with $\abs{X \oplus Y} > 1$, let $e_1, e_2, \cdots, e_i$ be edges in $X \setminus Y$ and let $f_1, f_2, \cdots, f_j$ be edges in $Y \setminus X$.
Construct following configuration path $P := (P_0, P_1, \cdots, P_{i + j})$ from $X$ to $Y$:
%\begin{align*}
%    \forall 0 \leq t \leq i + j, \quad P_t = \begin{cases}
%        X & \text{if } t = 0, \\
%        P_{t-1} \cup \{f_t\} & \text{if } 1 \leq t \leq j \\
%        P_{t-1} \setminus \{e_{t-j}\} & \text{if } t > j.
%    \end{cases}
%\end{align*}
\begin{itemize}
    \item let $P_0 = X$;
    \item for $1 \leq t \leq j$, let $P_t = P_{t-1} \cup \{f_t\}$;
    \item for $j < t$, let $P_t = P_{t-1} \setminus \{e_{t-j}\}$.
\end{itemize}
Note that $\abs{P_{t-1} \oplus P_{t}} = 1$ for all $1 \leq t \leq i + j$, and $P_t \in \+G$ for all $0 \leq t \leq i + j$.
Hence,
\begin{align*}
    \sum_{e\in E} \abs{\mu^X_e - \mu^Y_e}
    \leq \sum_{e \in E} \sum_{1 \leq t \leq i + j} \abs{\mu^{P_{t-1}}_e - \mu^{P_t}_e}
    = \sum_{1 \leq t \leq i + j} \sum_{e \in E} \abs{\mu^{P_{t-1}}_e - \mu^{P_t}_e}
    \leq \frac{\abs{X \oplus Y}}{2},
\end{align*}
where the last inequality follows from \eqref{eq:1-dist-decay} and the fact that $i + j = \abs{X \oplus Y}$.

%{\color{red}
\paragraph*{Verifying \Cref{item:good-event-2} of \Cref{cond:good-event-property}:}
Fix $S: E \to 2^E$, the random configuration $\sigma$ is generated by including each $e \in E$ independently with probability $\mu^{S(e)}_e$.
%The proof of the following lemma can be found in the proof of Lemma 5.5 in \cite{chen2023nearlinear}.

\begin{lemma}[\text{\cite[{Lemma 5.6}]{chen2023nearlinear}}] \label{lemma:marginal-bound}
    For any $T \subseteq E$ and $e \in E$, it holds that
    \begin{align*}
         \mu^T_e \geq 1 - 3(1-p_{\min})\log n.
    \end{align*}
\end{lemma}

For simplicity, let $K = (1 - p_{\min}) \log n$, and \Cref{lemma:marginal-bound} actually implies a marginal lower bound for $\sigma$, that is for each $e \in E$, $\Pr{e \in \sigma} \geq 1 - 3K$.

Since each edge $e$ is added to $\sigma$ independently, by the definition of $\+G$,
\begin{align*}
  \Pr{\sigma \not\in \+G}
  \le \sum_{S \in \+C} (3K)^{\abs{E(S,V \setminus S)}} 
  % &\text{(By \Cref{lm:st-dominate})}\\ 
  \le \sum_{S \in \+C} (3K)^{\abs{S} \log n} 
  % & \text{(definition of $\+C$)}\\
  \le \sum_{j=1}^{+\infty} n^j n^{j \log(3K)}
  \le n^{\log (27K)}.
\end{align*}
%
Recall that we choose 
\begin{align*}
    T^{\-{GD}} 
    &= \ctp{2m(\log m + \log(2/\epsilon))} \leq 4n^2 \log \tp{\frac{4n^2}{\epsilon}} \leq \frac{16n^4}{\epsilon} \leq \frac{n^{10}}{\epsilon},
\end{align*}
where in the last inequality, we use the assumption that $n \geq 3$.
By assumption, it holds that
\begin{align*}
    n^{\log(27K)} 
    &= \exp\tp{\log n \cdot \log (27K) } \\
    &\leq \exp\tp{\log n \cdot \log \tp{\-{e}^{-40} \exp\tp{- \frac{3\log(1/\epsilon)}{\log n}}}} \\
    &= \exp\tp{\log n \cdot \tp{-40 - \frac{3\log(1/\epsilon)}{\log n}}} \\
    &= \exp\tp{-40 \log n - 3\log(1/\epsilon)} = \frac{\epsilon^3}{n^{40}} \leq \frac{\epsilon}{16 T^{\-{GD}}},
\end{align*}
where in the last inequality, we use $n \geq 3$.
This finishes the verification. %of \Cref{item:good-event-2} of \Cref{cond:good-event-property}.
%}
\end{proof}

\iffalse % old verification of Item 2

\paragraph*{Verifying \Cref{item:good-event-2} of \Cref{cond:good-event-property}:}
Recall in \cref{alg:BP-simulation}, for $\ell \geq 1, 1\leq i \leq \tGD$, $Y^\ell_i$ is assigned as:
\begin{equation*}
Y^\ell_i=\left\{
\begin{aligned}
1 & \quad \randseed_i < \frac{\mu(\sigma^\ell_i \cup \{e_i\})}{\mu(\sigma^\ell_i \cup \{e_i\})+\mu(\sigma^\ell_i \setminus\{e_i\})} \\
0 & \quad \text{otherwise} 
\end{aligned}
\right.
%\nonumber
\end{equation*}
% where $\+R_i$ is picked from $[0, 1]$ u.a.r. and $\sigma^\ell_i \subseteq E$ is constructed as:
% \begin{align*}
% \forall e\in E, e\in \sigma^\ell_i \text{ iff. } Y^{\ell-1}_{j_e}=1, \text{where } j_e = \max\{j\geq 0 \mid e\in E_j\}.
% %\nonumber
% \end{align*}
We claim that $Y_i^\ell$ is assigned to $1$ with high probability under the current choice of parameters.
%{\color{red}
The proof of the following lemma can be found in the proof of Lemma 5.5 in \cite{chen2023nearlinear}.
%}
\begin{lemma}[\cite{chen2023nearlinear}] \label{lemma:marginal-bound}
    For any $S \subseteq E$ and $e \in E$, it holds that
    \begin{align*}
        \frac{\mu(S \cup \{e\})}{\mu(S \cup \{e\}) + \mu(S\setminus \{e\})} \geq 1 - 3(1-p_{\min})\log n.
    \end{align*}
\end{lemma}
%
For simplicity, let $K=(1-p_{\min}) \log n$. 
We first claim that for any $1 \le i \le \tPA$ and $1 \le \ell \le \tGD$, there exists a coupling of $\sigma^\ell_i$ and $U$ satisfying $U \subseteq \sigma^\ell_i$, where $U$ is formed by adding each element $e \in E$ into set $U$ with probability $1-3K$. We prove this by induction on $i$.

The induction basis $i=1$ follows from $\sigma_1^\ell = E$ for all $1 \le \ell \le \tGD$. Suppose that our claim holds for $i=j$. For any fixed $1 \le \ell \le \tGD$, by the definition of $\sigma_i^t$ and the updating rule of $Y_i^t$, 
\begin{equation*}
\sigma^\ell_{j+1}=\left\{
\begin{aligned}
\sigma^{\ell}_j \cup \{e_j\} & \quad \randseed_j < \frac{\mu(\sigma^{\ell-1}_j \cup \{e_j\})}{\mu(\sigma^{\ell-1}_j \cup \{e_j\})+\mu(\sigma^{\ell-1}_j \setminus\{e_j\})} \\
\sigma^{\ell}_j \setminus \{e_j\} & \quad \text{otherwise.} 
\end{aligned}
\right.
%\nonumber
\end{equation*}

By induction hypothesis, there exists a coupling $\mathcal{C}$ of $\sigma_j^{\ell}$ and $U$ satisfying $U \subseteq \sigma_j^{\ell}$. We construct a coupling of $\sigma_{j+1}^\ell$ and $U$ as follows:
\begin{enumerate}
\item draw $(\sigma_j^{\ell}, U') \sim \mathcal{C}$;
\item draw $e_j \in E$ and $\randseed_j \in [0,1]$ independently and uniformly at random;
\item set $\sigma^\ell_{j+1}=\sigma^{\ell}_j \cup \{e_j\}$ if $R_j < \frac{\mu(\sigma^{\ell-1}_j \cup \{e_j\})}{\mu(\sigma^{\ell-1}_j \cup \{e_j\})+\mu(\sigma^{\ell-1}_j \setminus\{e_j\})}$ and set $\sigma^\ell_{j+1}=\sigma^{\ell-1}_j \setminus \{e_j\}$ otherwise;
\item set $U = U' \cup \{e_j\}$ if $\randseed_j < 1-3K$, and set $U = U' \setminus \{e_j\}$ otherwise.
\end{enumerate}

By \cref{lemma:marginal-bound}, it holds that $U \subseteq \sigma^\ell_{j+1}$, concluding the proof of the claim.

Therefore, for any fixed $1 \le i \le \tPA, 1 \le t \le \tGD$, by the definition of $\+G$,
\begin{align*}
  \Pr{\sigma^t_i \not\in \+G} \le \Pr{U \not\in \+G} 
  \le \sum_{S \in \+C} (3K)^{\abs{E(S,V \setminus S)}} 
  % &\text{(By \Cref{lm:st-dominate})}\\ 
  \le \sum_{S \in \+C} (3K)^{\abs{S} \log n} 
  % & \text{(definition of $\+C$)}\\
  \le \sum_{j=1}^{+\infty} n^j n^{j \log(3K)}
  \le n^{\log (27K)}.
\end{align*}

Recall that we choose 
\begin{align*}
    T^{\-{GD}} 
    &= \ctp{2m(\log m + \log(4/\epsilon))} \leq 3n^2 \log \tp{\frac{4n^2}{\epsilon}} \leq \frac{12n^4}{\epsilon} \leq \frac{n^{10}}{\epsilon},
\end{align*}
where in the last inequality, we use the assumption that $n \geq 3$.
%Note that we also have
%\begin{align*}
%    T^{\-{PA}} \leq \frac{\-{e} T^{\-{GD}}}{m} + \log \frac{n}{\epsilon} + 3 \leq \frac{8n^4}{\epsilon} + \frac{2n}{\epsilon} \leq \frac{n^{10}}{\epsilon}.
%\end{align*}
%Now, in order to verify Item 2 of XXX, it is sufficient for us to verify that
%\begin{align*}
%    n^{\log(27K)} \leq \frac{\epsilon^3}{n^{30}} \leq \frac{\epsilon}{3 T^{\-{PA}} T^{\-{GD}}}.
%\end{align*}
By assumption, it holds that
\begin{align*}
    n^{\log(27K)} 
    &= \exp\tp{\log n \cdot \log (27K) } \\
    &\leq \exp\tp{\log n \cdot \log \tp{\-{e}^{-40} \exp\tp{- \frac{3\log(1/\epsilon)}{\log n}}}} \\
    &= \exp\tp{\log n \cdot \tp{-40 - \frac{3\log(1/\epsilon)}{\log n}}} \\
    &= \exp\tp{-40 \log n - 3\log(1/\epsilon)} = \frac{\epsilon^3}{n^{40}} \leq \frac{\epsilon}{16 T^{\-{GD}}},
\end{align*}
where in the last inequality, we use $n \geq 3$.
This finishes the verification of \Cref{item:good-event-2} of \Cref{cond:good-event-property}.

\fi 

% Now, we only left to prove \Cref{lemma:marginal-bound}.
% \begin{proof}[Proof of \Cref{lemma:marginal-bound}]
% For convenience, let $e = (u, v)$.
% We consider the following cases.
% \begin{enumerate}
%     \item $u, v$ are in the same connected component in graph $(V, S\setminus \{e\})$. In this case,
%     \begin{align*}
%         \frac{\mu(S \cup \{e\})}{\mu(S \cup \{e\}) + \mu(S \setminus \{e\})} = p_e \geq 1 - K/\log n \geq 1 - 3K.
%     \end{align*}
%     \item $u, v$ are in different connected components in graph $(V, S\setminus \{e\})$. In this case, let $C_u$ and $C_v$ to denote the connected conponents that contains $u$ and $v$, respectively. It holds that,
%     \begin{align*}
%         \frac{\mu(S \cup \{e\})}{\mu(S \cup \{e\}) + \mu(S \setminus \{e\})} 
%         &= \frac{p_e (1 + \*\lambda^{C_u \cup C_v})}{p_e (1 + \*\lambda^{C_u \cup C_v}) + (1 - p_e)(1 + \*\lambda^{C_u})(1 + \*\lambda^{C_v})} \\
%         &= \frac{p_e (1 + \*\lambda^{C_u \cup C_v})}{1 + \*\lambda^{C_u \cup C_v} + (1 - p_e)(\*\lambda^{C_u} + \*\lambda^{C_v})}
%         \geq \frac{p_e}{3 - 2p_e}.
%     \end{align*}
%     Recall that $P_e \geq 1 - \frac{K}{\log n} \geq 1 - K$.
%     Therefore, $\frac{\mu(S \cup \{e\})}{\mu(S \cup \{e\}) + \mu(S\setminus \{e\})} \geq \frac{1 - K}{1 + 2K} \geq 1 - 3K$. \qedhere
% \end{enumerate}
% \end{proof}

% \input{sec/convergence.tex}

% {\color{red}

%In \cite{chen2023nearlinear}, they proved the rapid mixing of Glauber dynamics under constraints in \Cref{thm:GD-correctness}.

% \begin{lemma}[\text{\cite[Theorem 5.1]{chen2023nearlinear}}] \label{lemma:GD-mixing}
%     If $n = \abs{V} \geq 3, \epsilon \in (0, 1)$, and $\*p \geq 1 - K/\log n$, where 
%     \begin{align*}
%          K \leq \min\left\{10^{-5} \exp\tp{-\frac{\log (16/\epsilon)}{\log n}}, \frac{1 - \lambda_{\max}}{27} \right\}
%         \text{ and }
%         T^{\-{GD}} = \ctp{2m(\log m + \log(4/\epsilon))},
%     \end{align*}
%     then it holds that
%     \begin{align*}
%         \DTV{X_{T^{\-{GD}}}}{\mu} \leq \epsilon / 2.
%     \end{align*}
% \end{lemma}

% {\color{red}

% }

%The following result shows that \Cref{alg:BP-simulation} faithfully simulates the Glauber dynamics.

%{\color{red}
%In this paper, we will show that \Cref{alg:BP-simulation} faithfully simulates the Glauber dynamics. Before stating this result, we first present the following criterion, which states that the distance between a random pair of configuration ``almost surely'' decays after a step of Glauber dynamics. We note that this condition, as a variant of the one in \cite{hayes2006coupling}, also covers a large class of problems where the coupling from stationary technique \cite{hayes2006coupling} could be applied.
%}

%\begin{condition}
%\label{cond:good-event-property}
%{\color{red}
%Given parameter $\epsilon \in (0,1)$,
%}
%there exists $\G \subseteq 2^E$ satisfying the following conditions.
%\begin{enumerate}
%    \item 
%    \label{item:good-event-1}
%    For any $X,Y \in \G$, it holds that
%    $$\sum_{e\in E} d(X,Y,e) \leq \frac{|X \bigoplus Y |}{2},$$
%    where $d(X,Y,e)=\left|\frac{\mu(X\cup \{e\})}{\mu(X\cup \{e\})+\mu(X\setminus\{e\})}-\frac{\mu(Y\cup \{e\})}{\mu(Y\cup \{e\})+\mu(Y\setminus\{e\})}\right|$.
%    %\item 
%    %\label{item:good-event-2}
%    %In \cref{alg:BP-simulation}, take the randomness over update sequence 
%    %$\R$,
%    %%$\R=\left((e_1,\randseed_1),(e_2,\randseed_2),...,(e_{\tGD},\randseed_{\tGD}) \right)$ where each $(e_i,\randseed_i)\in E\times [0,1]$ chosen uniformly and independently at random, 
%    %for each $1\leq \ell \leq \tPA, 1\leq i \leq \tGD$, the probability $\sigma^\ell_i \notin \G$ is at most $\delta$, where $\delta = \epsilon/(16\tGD)$.
%    \item
%    \label{item:good-event-2}
%    For $1\leq t \leq \tPA, 1\leq i \leq \tGD$, the probability $\sigma^t_i \notin \G$ in \cref{alg:BP-simulation} is at most $\delta = \frac{\epsilon}{16\tGD}$.
%
%    %TODO: $\sigma^\ell_i$ is not defined in \cref{alg:BP-simulation}.
%    %$\epsilon/(3\tPA\tGD)$
%\end{enumerate}
%\end{condition}

%\begin{theorem} \label{thm:dtv-xALG-GD}
%    If \Cref{cond:good-event-property} holds, then it holds that
%    \begin{align*}
%    \Pr{\xALG \neq X_{\tGD}} \leq \epsilon / 2.
%    \end{align*}
%\end{theorem}

%{\color{red} \Cref{thm:dtv-xALG-GD} will be proved in XXX.}
%
%Now, \Cref{thm:GD-correctness} could be proved by using \Cref{lemma:GD-mixing} and \Cref{thm:dtv-xALG-GD}, where each of them ccontributes an error of $\epsilon / 2$.
%The only non-trivial part is to verfy \Cref{cond:good-event-property}.

%\begin{lemma} \label{lemma:verify-cond-GD-sim}
%    Under the assumption of \Cref{thm:GD-correctness}, \Cref{cond:good-event-property} holds with $\eta = \frac{\epsilon}{16\tGD}$.
%\end{lemma}
%
%
%The proof of \Cref{thm:dtv-xALG-GD} and \Cref{lemma:verify-cond-GD-sim} will be given in \Cref{sec:dtv-xALG-GD} and \Cref{sec:verify-cond-GD-sim}, respectively.
%We remark that \Cref{thm:dtv-xALG-GD} is our main technical contribution in this paper, which guarantees the correctness of our parallel simulation of the Glauber dynamics under \Cref{cond:good-event-property}.
%
%Now, we are ready to prove \Cref{thm:GD-correctness}.

% }

==> sec/proof.tex <==
\begin{proof}[Proof of \Cref{lemma:correctness}]
%
  Without loss of generality, we assume that $\abs{V} > N_0$.
  %
   For $0 \le t \le T^{\mathrm{FD}}$, let $X_t$ be the configuration $X$ after the $t$-th iteration of \Cref{alg:field}, and let $Y_t$ be the 
   configuration $Y$ after the $t$-th iteration of the field dynamics $P^{\mathrm{FD}}_\theta$ starting from the same initial state $X_0=Y_0=E$.
   
   %We write 
   Let
   $\mu=\mu^{\-{RC}}_{E, \*p, \*\lambda}$ for short.
   By triangle inequality and the coupling lemma, it holds that
   \[
     \DTV{X_{T^{\-{FD}}}}{\mu}
     \leq \DTV{X_{T^{\-{FD}}}}{Y_{T^{\-{FD}}}} + \DTV{Y_{T^{\-{FD}}}}{\mu}
     \leq \Pr{X_{T^{\-{FD}}} \neq Y_{T^{\-{FD}}}} + \DTV{Y_{T^{\-{FD}}}}{\mu},
   \]
  %Note that $X_{T^{\-{FD}}} \neq Y_{T^{\-{FD}}}$ is equivalent to that there exists $1 \leq i \leq T^{\-{FD}}$ such that $X_i \neq Y_i$ but $X_j = Y_j$ for all $j < i$.
  for any coupling $(X_t,Y_t)$ of the two processes $X_t$ and $Y_t$.
  %
  And it is obvious that if $X_{T^{\-{FD}}} \neq Y_{T^{\-{FD}}}$, then there must exist $1 \leq i \leq T^{\-{FD}}$ such that $X_i \neq Y_i$ but $X_j = Y_j$ for all $0\le j < i$.
  %  By union bound, we have
  Hence, it holds that
  \begin{align*}
     \Pr{X_{T^{\-{FD}}} \neq Y_{T^{\-{FD}}}}
     &\le \sum_{i=1}^{T^{\-{FD}}} \Pr{X_i \neq Y_i \text{ and } \forall j < i, X_j = Y_j} 
     \leq \sum_{i=1}^{T^{\-{FD}}} \Pr{X_i \neq Y_i \mid X_{i-1} = Y_{i-1}}.
     %\leq \sum_{i=1}^{T^{\-{FD}}} \Pr{X_i \neq Y_i \mid \forall j < i, X_j = Y_j},
     %(\text{Markov chain}) \quad
     %&= \sum_{i=1}^{T^{\-{FD}}} \Pr{X_i \neq Y_i \mid X_{i-1} = Y_{i-1}},
   \end{align*}
    %For any $1 \le i \le T^{\-{FD}}$, consider the following coupling of $X_i$ and $Y_i$ condition on $X_{i-1} = Y_{i-1}$:
    For any $1 \le i \le T^{\-{FD}}$, conditioned on $X_{i-1} = Y_{i-1}$, we construct a coupling of $X_i$ and $Y_i$:
    \begin{enumerate}
      \item generate a random $S\subseteq E$ by adding each $e \in E$ independently with probability $\theta$;
      \item generate $(X_i, Y_i)$ according to the optimal coupling of $\widehat{\mu}^{\-{RC}}_{U,\*p^\star,\*\lambda}$ and $\mu^{\-{RC}}_{U,\*p^\star,\*\lambda}$, where $U = S \cup X_{i-1}$ and $\widehat{\mu}^{\-{RC}}_{U,\*p^\star,\*\lambda}$ is the distribution of the output of $\ParGD{(V, U)} {\*p^\star}{\*\lambda}{(2T^{\-{FD}})^{-1}\epsilon}$.
    \end{enumerate}
  %  A set $S \subseteq E$ is generated first, then $X_i = A(S)$ is generated by Resample$((V, S), \*p^\star, \*\lambda, (2T^{\-{FD}})^{-1}\epsilon)$ and $Y_i$ is generated according to the distribution $\mu^{\-{RC}}_{S, \*p^\star, \*\lambda}$.
  %  Consider the one-step optimal c It holds that
  By the coupling lemma and the assumption of \Cref{lemma:correctness}, it holds that
  \begin{align*}
     \Pr{X_i \neq Y_i \mid X_{i-1} = Y_{i-1}} &\leq \max_{U \subseteq E} \DTV{\widehat{\mu}^{\-{RC}}_{U,\*p^\star,\*\lambda}}{\mu^{\-{RC}}_{U, \*p^\star, \*\lambda}} \le \frac{\epsilon}{2T^{\mathrm{FD}}}.
   \end{align*}
   By \Cref{lemma:mixing-field} and our choice of $T^{\-{FD}}$, we have
   \begin{align*}
   \DTV{X_{T^{\-{FD}}}}{\mu} &\leq T^{\-{FD}} \frac{\epsilon}{2 T^{\-{FD}}} + \frac{\epsilon}{2} = \epsilon. %\qedhere
   \end{align*}
\end{proof}

Now, it only remains to prove \Cref{lemma:GD-sim-correctness}.

\begin{proof} [Proof of \Cref{lemma:GD-sim-correctness}]
    It is sufficient to verify the condition of \Cref{thm:GD-correctness} with error bound $\frac{\epsilon}{2\tFD}$ on the new instance $\mu^{\-{RC}}_{U,\*p^\star, \*\lambda}$:
    \begin{align} \label{eq:cond-gd-mix}
        (1 - p^\star_{\min}) \log n \leq \min\left\{\-{e}^{-40} \exp\tp{-\frac{5\log (2 T^{\-{FD}}/\epsilon)}{\log n}}, \frac{1 - \lambda_{\max}}{27} \right\}.
    \end{align}
 %   {\color{red}
    By our assumption $n \ge N_0 \ge \max \left\{4,\frac{3}{p_{\min}}, {\color{black} \sqrt{\frac{\log \tp{2/\epsilon^2}}{\log n}} } \right\}$, it holds that
 %   }
    \begin{align} 
        % \nonumber
        \log T^{\mathrm{FD}} 
        %&\le {5(1-\lambda_{\max})^{-2}} \log \tp{\frac{\e \log n}{K p_{\min}}} + \log \tp{2 \log n + \log \log \frac{2}{p_{\min}} + \log \frac{2}{\epsilon^2}} + 1\\
        %
        \label{eq:TFD-ub}
        \le 6(1-\lambda_{\max})^{-2} \log \tp{1/K} + 14(1-\lambda_{\max})^{-2} \log n,
    \end{align}
    where for convenience, we denote 
 %   {\color{red}
    \begin{align*}
        K := \theta \cdot \frac{\log n}{p_{\min}} = \e^{-100} \exp\tp{\frac{10\log(\epsilon/2)}{\log n}} \exp\tp{-140(1 - \lambda_{\max})^{-2}}.
    \end{align*}
 %   }
    %We remark that the upper bound of $T^{\-{FD}}$ is also used in the proof of Theorem 1.3 in~\cite{chen2023nearlinear}.
    %
    %First, note that  
    The first term in the right hand side of \eqref{eq:cond-gd-mix} can be bounded by
 %   {\color{red}
    \begin{align*}
        \e^{-40} \exp&\tp{-\frac{5\log (2 T^{\-{FD}}/\epsilon)}{\log n}} 
        = \e^{-40} \exp\tp{-\frac{5\log T^{\-{FD}}}{\log n} + \frac{5\log(\epsilon/2)}{\log n}}  \\
        %
        % &\geq \e^{-50} \epsilon^5 \exp\tp{-\frac{5\log T^{\-{FD}}}{\log n}} \\
        %
        (\text{by \eqref{eq:TFD-ub}}) \quad
        &\geq \e^{-50} \exp\tp{\frac{5\log(\epsilon/2)}{\log n}} \exp\tp{-70 (1 - \lambda_{\max})^{-2} +\frac{30(1 - \lambda_{\max})^{-2}\log K}{\log n}} \\
        %
        &\geq \e^{-50} \exp\tp{\frac{5\log(\epsilon/2)}{\log n}} \exp\tp{-70 (1 - \lambda_{\max})^{-2}} K^{1/2},
    \end{align*}
 %   }
    where the last inequality holds since $n \geq N_0 \geq \exp\tp{60 (1 - \lambda_{\max})^{-2}}$.
    
    Note that the $\*p^\star= \frac{\*p}{\*p+\theta (1-\*p)}$ constructed in \Cref{alg:field} satisfies
    \begin{align*}
        p^{\star}_{\min} = \min_{e \in E} p^{\star}_e = \frac{p_{\min}}{p_{\min}+\theta (1-p_{\min})} \ge \frac{\log n}{\log n+K} \ge 1- \frac{K}{\log n}.
    \end{align*}
    Therefore, we have the following two bounds on $(1 - p^\star_{\min}) \log n$:
 %   {\color{red}
    \begin{align}
        \nonumber
        \tp{1-p^{\star}_{\min}} \log n \le K &\le \e^{-50}\exp\tp{\frac{5\log(\epsilon/2)}{\log n}}\exp\tp{-70(1-\lambda_{\max})^{-2}} K^{1/2} \\
        \label{eq:p1}
        &\le  \e^{-40} \exp\tp{-\frac{5\log (2 T^{\-{FD}}/\epsilon)}{\log n}}, \\
        \label{eq:p2}
        \tp{1-p^{\star}_{\min}} \log n \le K &\le \exp \tp{-140(1-\lambda_{\max})^{-2}} \le \frac{(1-\lambda_{\max})^2}{140} \le \frac{1-\lambda_{\max}}{27}.
    \end{align}
 %   }
    Combining ~\eqref{eq:p1} and ~\eqref{eq:p2}, we conclude the proof of \Cref{lemma:GD-sim-correctness}.
\end{proof}

==> sec/warp_up.tex <==
\section{Wrapping up} \label{sec:wrap-up}
We now prove \Cref{thm:field-sim}.
The \Cref{item:field-efficiency} (efficiency) of \Cref{thm:field-sim} will be proved in \Cref{sec:field-efficiency},
and \Cref{item:field-correctness} (accuracy)  of \Cref{thm:field-sim} will be proved in \Cref{sec:field-correctness}.


\subsection{Efficiency} \label{sec:field-efficiency}

%In this section, we will prove \Cref{item:field-efficiency} of \Cref{thm:field-sim}. We have the following result.

We first bound the efficiency of \Cref{alg:BP-simulation}, assuming the setting of parameters in \cref{tabel:parameters}.
\begin{proposition}
\label{pro:BP-running-time}
%Take the parameters given in \cref{tabel:parameters}, 
\Cref{alg:BP-simulation} teriminates in $O(\tPA\cdot\log m)$ parallel time steps on $O(m\cdot \tGD)$ machines.
\end{proposition}

\begin{proof}%[Proof of \cref{pro:BP-running-time}]
    %The parallel running time and the number of machines used in \cref{alg:BP-simulation} is dominated by \cref{line:sigma} and \cref{line:weight}. In \cref{line:sigma}, for each $e \in E$, $j_e$ is taken as maximum value of $j$ satisfying $j<i \textbf{ and } e\in E_j$, which can be computed in $O(\log \tGD)$-parallel time using $O(\tGD)$ machines by the standard divide and conquer approach, hence the construction of $\sigma$ in \cref{line:sigma} take $O(\log \tGD)$-parallel time using $O(m \cdot \tGD)$ machines.
    The parallel complexity of \cref{alg:BP-simulation} is dominated by \cref{line:pred} and \cref{line:weight}. 
    
    \cref{line:pred} requires to compute $\pred_i(e)=\max\{j\ge 1\mid j<i \land e_j=e \}\cup\{0\}$ for each $1\leq i\leq \tGD$ and $e\in E$ in parallel. For each edge $e\in E$, the update list $\lis_e$ is defined as: %follow:
    \begin{align}
        %\lis_e := \{ j\geq 1 \mid e_j=e\}
        \lis_e := \{ j\geq 1 \mid e_j=e\}\cup\{0\}
        \label{eq:upd-list}
    \end{align}
    To implement \cref{line:pred}, for each $e\in E$, we first store a sorted update list $\lis_e$ using parallel merge sort \cite{cole1988parallel}, which costs $O(\log \tGD)$ parallel time on $O(\tGD)$ machines.
    Then each predecessor $\pred_i(e)$ can be computed in $O(\log \tGD)$ parallel time on $O(1)$ machines by a binary search on sorted $\lis_e$. The whole process costs $O(\log \tGD)$ parallel time on $O(m \cdot \tGD) %= O(m^2(\log m+\log (1/\epsilon)))
    $ machines in total.
    
    %hence the construction of $\sigma$ in \cref{line:sigma} take $O(\log \tGD)$-parallel time using $O(m \cdot \tGD)$ machines.
    
    In \cref{line:weight}, the marginal distribution $\mu_{e_i}^\sigma=\frac{\mu(\sigma\cup\{e_i\})}{\mu(\sigma\cup\{e_i\})+\mu(\sigma\setminus \{e_i\})}=\frac{w(\sigma\cup\{e_i\})}{w(\sigma\cup\{e_i\})+w(\sigma\setminus \{e_i\})}$ 
    can be computed by calculating the weights of $\sigma\cup\{e_i\}$ and $\sigma\setminus\{e_i\}$ (defined in \eqref{eq:RC-weight}), whereas each weight can be computed by a connected component algorithm such as \cite{shiloach1980log}, which costs $O(\log m)$ parallel time on $O(n+m)$ machines. 
    Thus, each iteration of \cref{line:iter} costs $O(\log m)$ parallel time on $O(m \cdot \tGD) %=O(m^2(\log m+\log (1/\epsilon)))
    $ machines, and these $O(m \cdot \tGD)$ machines can be re-used in the next iteration. 
    In \cref{line:ini-X}, the marginal distribution $\mu_e^E$ can be computed in the same method, which costs $O(\log m)$ parallel time on $O(n+m)$ machines for each edge $e\in E$.
    
    For other costs, the preprocessing part (from \cref{line:ini1} to \cref{line:ini2}) of \cref{alg:BP-simulation} can be computed in $O(1)$ parallel time on $O(\tGD)%=O(m\log m)
    $ machines; and in \cref{line:res}, the result $X$ of \cref{alg:BP-simulation} can be computed in $O(1)$ parallel time on $O(m)$ machines, since $j_e$ is maximum of the sorted list $\lis_e$.

    Overall, %due to the choice of $\tPA=\ctp{3 \log \tp{\frac{8\tGD\tFD}{\epsilon}}}$, 
    \Cref{alg:BP-simulation} runs in $O(\tPA \cdot \log m)$ parallel time on $O(m \cdot \tGD)$ machines.
    %Overall, due to the choice of $\tPA=\ctp{3 \log \tp{\frac{8\tGD\tFD}{\epsilon}}}$, \Cref{alg:BP-simulation} takes $O(\log m\cdot \log(\tGD\tFD/\epsilon))$ parallel time using $O(m \cdot \tGD)$ machines.
\end{proof}


\begin{proof}[Proof of \Cref{item:field-efficiency} of \Cref{thm:field-sim}]
    When $\abs{V} \leq N_0$, \Cref{alg:field} generates $X$ by brute force, which costs $2^{O(N_0^2)} = \exp\tp{O_\delta\tp{\frac{\log(1/\epsilon)}{\log n}}}$  in total work.
    When $\abs{V} > N_0$, \Cref{alg:field} terminates within $\tFD$ iterations, and in each iteration, it generates a random $S$ using $O(1)$ parallel time on $O(m)$ machines and calls \Cref{alg:BP-simulation}.
    By \Cref{pro:BP-running-time}, we have that \Cref{alg:field} terminates within
 %   \begin{align*}
 %      {\color{red}
        $O(\tPA\cdot \log m) \cdot \tFD = \tp{\exp\tp{\frac{\log(1/\epsilon)}{\log n}} \cdot \log n}^{O_{\delta}(1)}$
 %      }
 %   \end{align*}
    parallel time steps on $O(m \cdot \tGD) = O_{\delta}(m^2\log(n/\epsilon))$ machines.
\end{proof}

%\begin{corollary}
%Take the parameters given in \cref{tabel:parameters}, 
%\Cref{alg:field} takes $(\epsilon^{-1} \cdot p_{\min}^{-1} \cdot \log n)^{O((1 - \lambda_{\max})^{-4})}$-parallel time using $O(n^6\log^2(n/\epsilon))$ machines.
%\end{corollary}


\subsection{Accuracy of sampling} \label{sec:field-correctness}
We now prove \Cref{item:field-correctness} of \Cref{thm:field-sim}, the accuracy of sampling of \Cref{alg:field}, still assuming the setting of parameters in \cref{tabel:parameters}.
%
A key step has already been provided in \Cref{thm:GD-correctness}.
%
To complete the proof, we are going to establish the followings.

\begin{lemma}\label{lemma:correctness}
  %Assuming the procedure $\ParGD{G}{\p}{\*\lambda}{\epsilon}$ outputs a random configuration $X$ satisfying $d_{\mathrm{TV}}(X,\mu^{\mathrm{RC}}_{E,\*p,\*\lambda}) < \epsilon$, then \Cref{alg:field} returns a random configuration $X$ with $d_{\mathrm{TV}}(X,\mu^{\mathrm{RC}}_{E,\*p,\*\lambda}) < \epsilon$.
   %
   %If in each call of $\ParGD{G}{\p}{\*\lambda}{\epsilon}$ (\Cref{alg:BP-simulation}) in \Cref{alg:field}, the output random configuration $X$ of it always satisfying $\DTV{X}{}$
   %
   If for every $U \subseteq E$, the output  $Y$ of $\ParGD{(V, U)}{\*p^\star}{\*\lambda}{(2\tFD)^{-1}\epsilon}$ always satisfies $\DTV{Y}{\mu^{\-{RC}}_{U, \*p^\star, \*\lambda}} \leq (2\tFD)^{-1}\epsilon$, 
   then the output $X$ of \Cref{alg:field} satisfies $\DTV{X}{\mu^{\-{RC}}_{E, \*p, \*\lambda}} \leq \epsilon$.
\end{lemma}

\begin{lemma} \label{lemma:GD-sim-correctness}
    %Let $\xALG$ be the output of GD-simulation$((V, U), \*p^\star, \*\lambda, (2T^{\-{FD}})^{-1}\epsilon)$, it holds that 
    Assuming $n=|V|\ge N_0$,
    it holds that for every $U \subseteq E$, the output $Y$ of the subroutine $\ParGD{(V, U)}{\*p^\star}{ \*\lambda}{(2T^{\-{FD}})^{-1}\epsilon}$ satisfies 
    \begin{align*}
        \DTV{Y}{\mu^{\-{RC}}_{U, \*p^\star, \*\lambda}} \leq \frac{\epsilon}{2 T^{\-{FD}}}.
    \end{align*}
\end{lemma}

\Cref{item:field-correctness} of \Cref{thm:field-sim} follows directly by combining \Cref{lemma:correctness} and \Cref{lemma:GD-sim-correctness}. 

\Cref{lemma:correctness} follows from the rapid mixing of the field dynamics.
\begin{lemma}[\text{\cite[Lemma 3.5]{chen2023nearlinear}}]\label{lemma:mixing-field}
  The mixing time of the field dynamics satisfies
  % Let $(X_t)_{t \in \mathbb{N}}$ be the field dynamics with parameter $\theta \in (0, 1)$, starting from $X_0 = E$ on the distribution $\mu^{\-{RC}}_{E, \*p, \*\lambda}$.
  % Now, suppose 
  \begin{align*}
    \forall \epsilon \in (0,1), \quad T_{\mathrm{mix}}(\epsilon) \leq \tp{\frac{\mathrm{e}}{\theta}}^{5(1-\lambda_{\max})^{-2}}\tp{2 \log n + \log \log \frac{2}{p_{\min}} + \log \frac{1}{2\epsilon^2}}.
  \end{align*}
  % then it holds that $\DTV{X_T}{\mu^{\-{RC}}_{E, \*p, \*\lambda}} \leq \epsilon$, where $n$ is the number of vertices.
\end{lemma}
